A distributed block coordinate descent method for training $l_1$ regularized linear classifiers

Distributed training of $l_1$ regularized classifiers has received great attention recently. Most existing methods approach this problem by taking steps obtained from approximating the objective by a quadratic approximation that is decoupled at the individual variable level. These methods are designed for multicore and MPI platforms where communication costs are low. They are inefficient on systems such as Hadoop running on a cluster of commodity machines where communication costs are substantial. In this paper we design a distributed algorithm for $l_1$ regularization that is much better suited for such systems than existing algorithms. A careful cost analysis is used to support these points and motivate our method. The main idea of our algorithm is to do block optimization of many variables on the actual objective function within each computing node; this increases the computational cost per step that is matched with the communication cost, and decreases the number of outer iterations, thus yielding a faster overall method. Distributed Gauss-Seidel and Gauss-Southwell greedy schemes are used for choosing variables to update in each step. We establish global convergence theory for our algorithm, including Q-linear rate of convergence. Experiments on two benchmark problems show our method to be much faster than existing methods.

==> Experiments_old.tex <==
\section{Experimental Evaluation}

In this section, we present experimental results on real-world datasets. We compare our methods with several state of the art methods, in particular, those analyzed in section 4 (see the methods in the first column of Table 3) together with \admm, the accelerated alternating direction method of multipliers~\citep{goldstein2013}. 
To the best of our knowledge, such a detailed study has not been done for parallel and distributed $l_1$ regularized solutions in terms of (a) accuracy and solution optimality performance, (b) variable selection schemes, (c) computation versus communication time and (d) solution sparsity. The results demonstrate the effectiveness of our methods in terms of total (computation + communication) time on both accuracy and objective function measures.

\subsection{Experimental Setup}

\noindent{\bf Datasets:} We conducted our experiments on two popular benchmark datasets \textsc{KDD} and \textsc{URL}\footnote{{\small See \url{http://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets/}. We refer to kdd2010 (algebra) dataset as \textsc{KDD}.}}. \textsc{KDD} has $n=8.41M$, $m=20.21M$ and $nz=0.31B$. \textsc{URL} has $n=2.00M$, $m=3.23M$ and $nz=0.22B$.
%the statistics are given in Table~\ref{tab:params}. 
These datasets have sufficiently interesting characteristics of having a large number of examples and features such that (1) feature partitioning, (2) $l_1$ regularization and (3) communication are important. \vspace*{0.05in}


%\noindent{\bf Methods for Comparison:}
%The methods that we implemented and studied are: (1)\textsc{ADMM}: accelerated alternating direction method of multipliers~\cite{gold2013}, (2) \textsc{Hyd}: HYbriD cooRdinAte descent method~\cite{richtarik2013a}, (3) \textsc{GRock}: Greedy coOrdinate-bl\textit{ock}~\cite{peng2013}, (4) \textsc{FPA}: Flexible Parallel Algorithm~\cite{facchinei2013}, (5) \textsc{PCD}: Parallel Coordinate Descent Newton method~\cite{bian2013} and (6) \textsc{DCD}: Distributed block Coordinate Descent - our method. We use these abbreviations for ease of reference in the plots and discussion below. We considered two variable selection rules, namely, random selection (R) and distributed Gauss-Southwell type rule (S) for our method and \textsc{PCD}~\cite{bian2013}. Random selection rule refers to random permutation of all variables in each outer iteration and blocks of specified working set size (WSS) are sequentially visited in each node as in Gauss-Seidel rule. We refer these variants as \textsc{DCD-R}, \textsc{DCD-S}, \textsc{PCD-R} and \textsc{PCD-S} with variable selection rule indicated after hyphenation. \vspace*{0.05in}

\noindent{\bf Methods and Metrics:} We evaluate the performance of all the methods using (a) Area Under Precision-Recall Curve (AUPRC)~\citep{alekh2013} and (b) Relative Function Value Difference (RFVD) as a function of time taken. RFVD is computed as $\log(\frac{F(w^t)-F^{*}}{F^{*}})$ where $F^{*}$ is taken as the best value obtained across the methods after a long duration. We stopped each method after 800 outer iterations. We also report per node computation time statistics and sparsity pattern behavior of all the methods. \vspace*{0.05in}

\noindent{\bf Parameter Settings:} We experimented with the $\lambda$ values of $(123,13.7,4.6) \times 10^{-7}$ and $(727,242,9) \times 10^{-8}$ for the \textit{KDD} and \textit{URL} datasets respectively. These values are chosen in such a way that they are centered around the respective optimal $\lambda$ value and have good sparsity variations over the optimal solution. With respect to Algorithm 1, the working set size (WSS) per node and number of nodes ($P$) are common across all the methods. We set WSS in terms of the fraction ($r$) of the number of features per node, i.e., WSS=$r\, m/P$. Note that WSS will change with $P$ for a given fraction $r$. For \textit{KDD} and \textit{URL}, we used three $r$ values $(0.01,0.1,0.25)$ and $(0.001,0.01,0.1)$ respectively. We experimented with $P = 25, 100$.
Also, $r$ does not play a role in ADMM since all variables are optimized in each node. \vspace*{0.05in}

\noindent{\bf Platform:} We ran all our experiments on a Hadoop cluster with $200$ nodes. Each node has Intel (R) Xeon (R) E5-2450L (2 processors) running at 1.8 GHz and 192 GB RAM. (Though both the datasets can fit in this memory configuration, our intention is to test the performance in a distributed setting.) All our implementations were done in $C\#$ including our binary tree \textit{AllReduce} support~\citep{alekh2013} on Hadoop.

%\subsection{Experimental Results}

\subsection{Method Specific Parameter Settings}

%\noindent{\bf Method Specific Parameter Settings:} 
We discuss method specific parameter setting used in our experiments and associated practical implications.

Let us begin with \admm. We use the feature partitioning formulation of ADMM described in section 8.3 of \citet{boyd2011}.
\admm~does not fit into the format of Algorithm 1, but the communication cost per outer iteration is comparable to the other methods that fit into Algorithm 1.
In \admm, the augmented Lagrangian parameter ($\rho$) plays an important role in getting good performance. In particular, the number of iterations required by ADMM for convergence is very sensitive with respect to $\rho$. While many schemes have been discussed in the literature~\citep{boyd2011} we found that selecting $\rho$ using the objective function value gave a good estimate; we selected $\rho^*$ from a handful of values with ADMM run for $10$ iterations (i.e., not full training) for each $\rho$ value tried.{\footnote{These initial ``tuning" iterations are not counted against the limit of 800 we set for the number of iterations. Thus, for ADMM, the total number of iterations can go higher than 800.} However, this step incurred some computational/communication time. In our time plots shown later, the late start of ADMM results is due to this cost. Note that this minimal number of iterations was required to get a decent $\rho^*$. \vspace*{0.05in}

\noindent{\bf Choice of ${\mathbf\mu}$ and ${\mathbf k}$:} To get a practical implementation that gives good performance in our method, we deviate slightly from the conditions of Theorem 1. First, we find that the proximal term does not contribute usefully to the progress of the algorithm (see the left side plot in Figure 1). So we choose to set $\mu$ to a small value, e.g., $\mu=10^{-12}$. Second, we replace the stopping condition (\ref{appopt}) by simply using a fixed number of cycles of coordinate descent to minimize $f_p^t$. The right side plot in Figure 1 shows the effect of number of cycles, $k$. We found that a good choice for the number of cycles is $10$ and we used this value in all our experiments.

For \grock, \fpa~and \richtarik~we set the constants $(L^j)$ as suggested in the respective papers. Unfortunately, we found \grock~to be either unstable and diverging or extremely slow. The left side plot in Figure~\ref{fig:Issues} depicts these behaviors. The solid red line shows the divergence case. \fpa~requires an additional parameter ($\gamma$) setting for the stochastic approximation step size rule. Our experience is that setting right values for these parameters to get good performance can be tricky and highly dataset dependent. The right side plot in Figure~\ref{fig:Issues} shows the extremely slow convergence behavior of \fpa. Therefore, we do not include \grock~and \fpa~further in our study.

\begin{figure}[t]
%\vspace{-1in}
\hspace{-0in}
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/mueffect-nodes-100.eps}
%\vspace{-0.08in}
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/inneriterations.eps}
%\vspace{-0.75in}
\caption{\small{Left: the effect of $\mu$. Right: the effect of $k$, the number of cycles to minimize $f^t_p$. $\mu = 10^{-12}$ and $k = 10$ are good choices. $P=100$.}}
\label{fig:MuPlot}
\vspace{-0.15in}
\end{figure}

\begin{figure}[t]
%\vspace{-1in}
\hspace{-0in}
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/grockplot-data-url-lambda-2pt424689e-06-nodes-25.eps}
%\vspace{-0.08in}
%\hspace{-0.08in}
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/fpaplot-data-kdd-lambda-4pt585581e-07-nodes-100.eps}
%\vspace{-0.75in}
\caption{\small{Left: Divergence and slow convergence of \grock~on the \textsc{URL} dataset ($\lambda = 2.4 \times 10^{-6}$ and $P = 25$). Right: Extremely slow convergence of \fpa~on the \textsc{KDD} dataset ($\lambda = 4.6 \times 10^{-7}$ and $P = 100$).}}
\label{fig:Issues}
\vspace{-0.15in}
\end{figure}


\subsection{Performance Evaluation}

We begin by comparing the efficiency of various methods and demonstrating the superiority of the new methods that were motivated in section 4 and developed in section 5. After this we analyze and explain the reasons for the superiority. \vspace*{0.05in}

\noindent{\bf Study on AUPRC and RFVD:} 
We compare the performance of all methods by studying the variation of AUPRC and RFVD as a function of time, for various choices of $\lambda$, working set size (WSS) and the number of nodes ($P$) on \textsc{KDD} and \textsc{URL} datasets. To avoid cluttering with too many plots, we provide only representative ones; but, the observations that we make below hold for others too.

Figure~\ref{fig:kddobj} shows the objective function plots for (\textit{KDD}) with $\lambda$ set to $4.6 \times 10^{-7}$. We see that \dbcds~clearly outperforms all other methods; for example, if we set the RFVD value to $-2$ as the stopping criterion, \dbcds~is faster than existing methods by an order of magnitude. \pcdns~comes as the second best. The S-scheme gives significant speed improvement over the R-scheme.
As we compare the performance for two different WSS (see Figure~\ref{fig:kddobj}(a)(b)), larger WSS gives some improvement and this speed-up is significant for \richtarik, \pcdnr~and \dbcdr. Note that \admm~is WSS independent since all the variables are updated. Because all variables are updated, ADMM performs slightly better than \richtarik, \pcdnr~and \dbcdr~when WSS is small (see Figure~\ref{fig:kddobj}(a)(c)). In this case, other methods take some time to reach optimal values, when the working set is selected randomly using the R-scheme. If we compare \admm~and \dbcds, \admm~is inferior; this holds even if we leave out the initial time needed for setting $\rho$.


\begin{figure*}[t]
%\vspace{-1in}
\centering
\subfigure[$P = 25$, $WSS = 8086$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-kdd-workingset-8086-lambda-4pt585581e-07-nodes-25.eps}
\vspace*{-2in}
}
\subfigure[$P = 25$, $WSS = 80867$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-kdd-workingset-80867-lambda-4pt585581e-07-nodes-25.eps}
\vspace*{-2in}
}
\subfigure[$P = 100$, $WSS = 2021$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-kdd-workingset-2021-lambda-4pt585581e-07-nodes-100.eps}
\vspace*{-2in}
}
\subfigure[$P = 100$, $WSS = 20216$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-kdd-workingset-20216-lambda-4pt585581e-07-nodes-100.eps}
\vspace*{-2in}
}
%\vspace*{-0.75in}
\caption{\small{\textsc{KDD} dataset. Relative function value difference in log scale. $\lambda = 4.6 \times 10^{-7}$}}
\label{fig:kddobj}
\vspace{-0.15in}
\end{figure*}





\begin{figure*}[t]
%\vspace{-1in}
\centering
\subfigure[$P = 25$, $WSS = 1292$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-url-workingset-1292-lambda-8pt980331e-08-nodes-25.eps}
\vspace*{-2in}
}
\subfigure[$P = 25$, $WSS = 12927$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-url-workingset-12927-lambda-8pt980331e-08-nodes-25.eps}
\vspace*{-2in}
}
\subfigure[$P = 100$, $WSS = 323$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-url-workingset-323-lambda-8pt980331e-08-nodes-100.eps}
\vspace*{-2in}
}
\subfigure[$P = 100$, $WSS = 3231$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-url-workingset-3231-lambda-8pt980331e-08-nodes-100.eps}
\vspace*{-2in}
}
%\vspace*{-0.75in}
\caption{\small{\textsc{URL} dataset. Relative function value difference in log scale. $\lambda = 9.0 \times 10^{-8}$}}
\label{fig:urlobj}
\vspace{-0.15in}
\end{figure*}


\begin{figure*}[t]
\centering
\subfigure[$P = 25$, $WSS = 8086$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-kdd-workingset-8086-lambda-4pt585581e-07-nodes-25.eps}
}
\subfigure[$P = 25$, $WSS = 80867$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-kdd-workingset-80867-lambda-4pt585581e-07-nodes-25.eps}
}
\subfigure[$P = 100$, $WSS = 2021$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-kdd-workingset-2021-lambda-4pt585581e-07-nodes-100.eps}
}
\subfigure[$P = 100$, $WSS = 20216$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-kdd-workingset-20216-lambda-4pt585581e-07-nodes-100.eps}
}
%\vspace*{-0.2in}
\caption{\small{\textsc{KDD} dataset. AUPRC Plots. $\lambda = 4.6 \times 10^{-7}$}}
\label{fig:kddauprc}
\end{figure*}

\begin{figure*}[t]
\centering
\subfigure[$P = 25$, $WSS = 1292$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-url-workingset-1292-lambda-8pt980331e-08-nodes-25.eps}
}
\subfigure[$P = 25$, $WSS = 12927$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-url-workingset-12927-lambda-8pt980331e-08-nodes-25.eps}
}
\subfigure[$P = 100$, $WSS = 323$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-url-workingset-323-lambda-8pt980331e-08-nodes-100.eps}
}
\subfigure[$P = 100$, $WSS = 3231$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-url-workingset-3231-lambda-8pt980331e-08-nodes-100.eps}
}
%\vspace*{-0.2in}
\caption{\small{\textsc{URL} dataset. AUPRC plots. $\lambda = 9.0 \times 10^{-8}$}}
\label{fig:urlauprc}
\end{figure*}

\begin{figure*}[t]
\centering
\subfigure[\textsc{KDD}, $WSS = 2021$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-kdd-workingset-2021-lambda-1pt238107e-05-nodes-100.eps}
}
\subfigure[\textsc{KDD}, $WSS = 20216$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-kdd-workingset-20216-lambda-1pt238107e-05-nodes-100.eps}
}
\subfigure[\textsc{URL}, $WSS = 323$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-url-workingset-323-lambda-7pt274068e-06-nodes-100.eps}
}
\subfigure[\textsc{URL}, $WSS = 3231$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsobjfunc-data-url-workingset-3231-lambda-7pt274068e-06-nodes-100.eps}
}
%\vspace*{-0.2in}
\caption{\small{Relative function value difference in log scale. \textsc{KDD} dataset: $\lambda = 1.2 \times 10^{-5}$. \textsc{URL} dataset: $\lambda = 7.3 \times 10^{-7}$}}
\label{fig:kddurlobj}
\end{figure*}


\begin{figure*}[t]
\centering
\subfigure[\textsc{KDD}, $WSS = 2021$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-kdd-workingset-2021-lambda-1pt238107e-05-nodes-100.eps}
}
\subfigure[\textsc{KDD}, $WSS = 20216$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-kdd-workingset-20216-lambda-1pt238107e-05-nodes-100.eps}
}
\subfigure[\textsc{URL}, $WSS = 323$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-url-workingset-323-lambda-7pt274068e-06-nodes-100.eps}
}
\subfigure[\textsc{URL}, $WSS = 3231$]{
\includegraphics[width=0.45\linewidth]{plots/finalplotseps/timevsauprc-data-url-workingset-3231-lambda-7pt274068e-06-nodes-100.eps}
}
%\vspace*{-0.2in}
\caption{\small{AUPRC plots. \textsc{KDD} dataset: $\lambda = 1.2 \times 10^{-5}$. \textsc{URL} dataset: $\lambda = 7.3 \times 10^{-7}$}}
\label{fig:kddurlauprc}
\end{figure*}

Figure~\ref{fig:urlobj} shows the objective function plots for (\textit{URL}) with $\lambda$ set to $9 \times 10^{-8}$. Here again, \dbcds~gives the best RFVD performance with order of magnitude speed-up over existing methods. \richtarik~suffers slow convergence and \admm~gives a decent second best performance. Interestingly, the new variable selection rule (S-scheme) did not do very well for \pcdn~for large WSS. This shows that working with quadratic approximations (like \pcdns~does) can at times be quite inferior compared to using the actual nonlinear objective (like \dbcds~does). On comparing the performance for two different WSS, some speed improvement is achieved as in the case of \textsc{KDD} with similar observations. All these objective function progress behaviors are consistent with the AUPRC plots (Figures~\ref{fig:kddauprc} and \ref{fig:urlauprc}) as well except in one case. For example, the AUPRC performance of \pcdns~is quite good although it is a bit slow on the objective function.

Figures~\ref{fig:kddurlobj} and \ref{fig:kddurlauprc} show the performance plots for another choice of different $\lambda$ values for the datasets. \dbcds~gives the best performance on \textit{URL}. On \textit{KDD}, it is the second best after \pcdns. This happens because the $S$ scheme selects features having a large number of non-zero feature values. As a result, computation cost goes up a bit as we do more inner iterations compared to \pcdns. Nevertheless, the performance of \dbcds~is still very good. Overall, the results point to the choice of \dbcds~as the preferred method as it is highly effective with an order of magnitude improvement over existing methods. It is also worth noting that our proposal of using the S-scheme with the \pcdn~method~\citep{bian2013} offers significant value.

Next we analyze the reason behind the superior performance of \dbcds. It is very much along the motivational ideas laid out in section 4: since communication cost dominates computation cost in each outer iteration, \dbcds~reduces overall time by decreasing the number of outer iterations. 

\def\stap{{ {> 800} }}

%\vspace*{-0.2in}
\begin{table}[h]
\caption{$T^P$, the number of outer iterations needed to reach RFVD$\le \tau$, for various $P$ and $\tau$ values. Best values are indicated in boldface. (Note the $\log$ in the definition of RFVD.) Working set size is set at 1\% ($r=0.1$, $WSS=rm/P$). For each dataset, the $\tau$ values were chosen to cover the region where AUPRC values are in the process of reaching the steady state value.}
\label{tab:numiter}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\multicolumn{8}{c}{} \\
\multicolumn{8}{c}{KDD, $\lambda = 4.6\times 10^{-7}$} \\
\multicolumn{8}{c}{} \\
%\vspace*{0.1cm}
\hline
\multicolumn{2}{|c}{} & \multicolumn{3}{|c|}{Existing methods} & \multicolumn{3}{c|}{Our methods}   \\
\hline
P    &  $\tau$     &  \richtarik  &  \admm     &   \pcdnr   &   \pcdns     &  \dbcdr    & \dbcds    \\
\hline
     & $-1$        &  298         & 159        & 294        & 12           & 236        & {\bf 8}   \\
 25  & $-2$        & $\stap$      & 317        & $\stap$    & 311          & $\stap$    & {\bf 104} \\
     & $-3$        & $\stap$      & $\stap$    & $\stap$    & $\stap$      & $\stap$    & {\bf 509} \\
\hline
     & $-1$        & 297          & 180        & 299        & 12           & 230        & {\bf 10}  \\
 100 & $-2$        & $\stap$      & $\stap$    & $\stap$    & 311          & $\stap$    & {\bf 137} \\
     & $-3$        & $\stap$      & $\stap$    & $\stap$    & {\bf 650}    & $\stap$    & 668       \\
\hline
\multicolumn{8}{c}{} \\
\multicolumn{8}{c}{URL, $\lambda = 9.0\times 10^{-8}$} \\
\multicolumn{8}{c}{} \\
\hline
     & $0$         & 376          & 137        & 106        & 65           & 101        & {\bf 6}   \\
 25  & $-0.5$      & $\stap$      & 179        & 337        & 117          & 193        & {\bf 14}  \\
     & $-1$        & $\stap$      & 214        & 796        & 196          & 722        & {\bf 22}  \\
\hline
     & $0$         & 400          & 120        & 91         & 64           & 78         & {\bf 7}   \\
 100 & $-0.5$      & $\stap$      & 176        & 313        & 116          & 182        & {\bf 16}  \\
     & $-1$        & $\stap$      & 231        & 718        & 190          & 582        & {\bf 28}  \\
\hline
\end{tabular}
\end{center}
\end{table}

\noindent{\bf Study on the number of outer iterations:} 
We study $T^P$, the number of outer iterations needed to reach RFVD$\le \tau$. Table~\ref{tab:numiter} gives $T^P$ values for various methods in various settings. \dbcds~clearly outperforms other methods in terms of having much smaller values for $T^P$. \pcdns~is the second best method, followed by \admm. The solid reduction of $T^P$ by \dbcds~validates the design that was motivated in section 4. The increased computation associated with \dbcds~is immaterial; because communication cost overshadows computation cost in each iteration for all methods, \dbcds~is also the best in terms of the overall computing time. The next set of results gives the details. \vspace*{0.05in}

\noindent{\bf Computation and Communication Time:}
As emphasized earlier, communication plays an important role in the distributed setting. To study this effect, we measured the computation and communication time separately at each node. Figure~\ref{fig:comptime} shows the computation time per node on the \textit{KDD} dataset. In both cases, \admm~incurs significant computation time compared to other methods. This is because it optimizes over all variables in each node. \dbcds~and \dbcdr~come next because our method involves both line search and $10$ inner iterations. \pcdnr~and \pcdns~take a little more time than \richtarik~because of the line search. As seen in both \dbcd~and \pcdn~cases, a marginal increase in time is incurred due to the variable selection cost with the S-scheme compared to the R-scheme.

%\vspace*{-0.2in}
\begin{table}[h]
\caption{Computation and communication costs per iteration (in secs.) for KDD, $P=25$.}
\label{tab:timings}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c}
\hline
Method & Comp. & Comm. & Comp. & Comm.\\
\hline
& \multicolumn{2}{|c|}{WSS: $r=0.1$} & \multicolumn{2}{|c|}{WSS: $r=0.01$}\\
\hline
Hyd & 0.022 & 5.192 & 0.131 & 4.888\\
\hline
PCD-R & 0.138 & 5.752 & 0.432 & 5.817\\
\hline
PCD-S & 1.564 & 7.065 & 1.836 & 7.032\\
\hline
DBCD-R & 0.991 & 6.322 & 1.978 & 6.407\\
\hline
DBCD-S & 5.054 & 6.563 &  5.557 & 8.867\\
\hline
\end{tabular}
\end{center}
\end{table}


We measured the computation and communication time taken per iteration by each method for different $P$ and $WSS$ settings. From Table~\ref{tab:timings} (which gives representative results for one situation, \textsc{KDD} and $P=25$), we see that the communication time dominates the cost in \richtarik~and \pcdnr.
\dbcdr~takes more computation time than \pcdnr~and \richtarik~since we run through $10$ cycles of inner optimization. Note that the methods with S-scheme take more time; however, the increase is not significant compared to the communication cost. \dbcds~takes the maximum computation time and is quite comparable to the communication time. Recall our earlier observation of \dbcds~giving order of magnitude speed-up in the overall time compared to methods such as \richtarik~and \pcdnr~(see Figures 3-8). Though the computation times taken by \richtarik, \pcdnr~and \pcdns~are lesser, they need significantly more number of iterations to reach some specified objective function optimality criterion. As a result, these methods become quite inefficient due to extremely large communication cost compared to \textsc{DBCD}. All these observations point to the fact our \dbcd~method nicely trades-off the computation versus communication cost, and gives an excellent order of magnitude improvement in overall time. With the additional benefit provided by the S-scheme, \dbcds~clearly turns out to be the method of choice for the distributed setting. \vspace*{0.05in}

\noindent{\bf Sparsity Pattern:} To study weight sparsity behaviors of various methods during optimization, we computed the percentage of non-zero weights ($\rho$) as a function of outer iterations. We set the initial weight vector to zero. Figure~\ref{fig:sparse} shows similar behaviors for all the random (variable) selection methods. After a few iterations of rise they fall exponentially and remain at the same level. For methods with the S-scheme, many variables remain non-zero for some initial period of time and then $\rho$ falls a lot more sharply. It is interesting to note that such an initial behavior seems necessary to make good progress in terms of both function value and AUPRC (Figure~\ref{fig:kddurlobj}(a)(b) and Figure~\ref{fig:kddurlauprc}(a)(b)) In all the cases, many variables stay at zero after initial iterations; therefore, shrinking ideas can be used to improve efficiency. \vspace*{0.05in}
%We also computed the percentage of sparsity change that is based on the number of transitions made at a specified threshold ($10^{-10}$); see the bottom row in Figure 7. Note that the sharp peak that appears is correlated with the sharper drop in $sd$.

\noindent{\bf Remark on Speed up:}
Let us consider the RFVD plots corresponding to \dbcds~in Figures~\ref{fig:kddobj}~and~\ref{fig:urlobj}. It can be observed that the times associated with $P=25$ and $P=100$ for reaching a certain tolerance, say RFVD=-2, are close to each other. This means that using 100 nodes gives almost no speed up over 25 nodes, which may prompt the question: {\it Is a distributed solution really necessary?} There are two answers to this question. First, as we already mentioned, when the training data is huge\footnote{The \textsc{KDD} and \textsc{URL} datasets are really not huge in the {\it Big data} sense. In this paper we used them only because of lack of availability of much bigger public datasets.} and so {\it the data is generated and forced to reside in distributed nodes}, the right question to ask is not whether we get great speed up, but to ask which method is the fastest. Second, for a given dataset, if the time taken to reach a certain optimality tolerance is plotted as a function of $P$, it may have a minimum at a value different from $P=1$. In such a case, it is appropriate to choose a $P$ (as well as $WSS$) optimally to minimize training time. Many applications involve periodically repeated model training. For example, in Advertising, logistic regression based click probability models are retrained on a daily basis on incrementally varying datasets. In such scenarios it is worthwhile to spend time to tune parameters such as $P$ and $WSS$ in an early deployment phase to minimize time, and then use these parameter values for future runs.

It is also important to point out that the above discussion is relevant to distributed settings in which communication causes a bottleneck. If communication cost is not heavy, e.g., when the number of examples is not large and/or communication is inexpensive such as in multicore solution, then good speed ups are possible; see, for example, the results in~\citet{richtarik2013}.


\begin{figure}[t]
\subfigure[$WSS = 2021$]{
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/comptimevsobjfunc-data-kdd-workingset-2021-lambda-1pt238107e-05-nodes-100.eps}
}
\subfigure[$WSS = 20216$]{
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/comptimevsobjfunc-data-kdd-workingset-20216-lambda-1pt238107e-05-nodes-100.eps}
}
%\vspace*{-0.2in}
\caption{\small{Per-node computation time on the \textsc{KDD} dataset ($\lambda = 1.2 \times 10^{-5}$ and $P = 100$).}}
\label{fig:comptime}
\end{figure}

\begin{figure}[t]
\subfigure[$WSS = 2021$]{
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/itersvssparsity-data-kdd-workingset-2021-lambda-1pt238107e-05-nodes-100.eps}
}
%\vspace{-0.08in}
\subfigure[$WSS = 20216$]{
\includegraphics[width=0.48\linewidth]{plots/finalplotseps/itersvssparsity-data-kdd-workingset-20216-lambda-1pt238107e-05-nodes-100.eps}
}
%\vspace{-0.08in}
%\includegraphics[width=0.48\linewidth]{plots/finalplotspdf/itersvssparsitychange-data-kdd-workingset-2021-lambda-1.23811e-005-nodes-100.pdf}
%\vspace{-0.08in}
%\hspace{-0.08in}
%\includegraphics[width=0.48\linewidth]{plots/finalplotspdf/itersvssparsitychange-data-kdd-workingset-20216-lambda-1.23811e-005-nodes-100.pdf}
%\vspace*{-0.2in}
\caption{\small{\textsc{KDD} dataset: Percentage of non-zero weights. $\lambda = 1.2 \times 10^{-5}$ and $P = 100$. }}
\label{fig:sparse}
\end{figure}








==> rw.tex <==

\section{Related Work}

There exists a large volume of literature addressing the problem of optimizing $L1$ regularized objective functions~(see for e.g., \cite{lee2006,andrew2007,yun2011,beck2009,yuan2012,yuan2010}). The aspects in which the methods proposed therein differ include: (i) applications (e.g., compressed sensing and high dimensional classification/regression) to exploit any structure, (ii) assumptions made on the loss functions (e.g., convex/non-convex, squared error/hinge loss, smooth/non-smooth, decomposable, etc), (iii) computing environment (single, parallel, distributed) and (iv) algorithmic (details given below). We are interested in building high dimensional linear classifiers with convex and smooth loss functions. 

In the computing environment aspect, there are several algorithms that focus on doing parallel computations in a single machine having multi-cores (see~\cite{bradley2011}, \cite{richtarik2013}, \cite{bian2013}, \cite{peng2013}). In this scenario, memory is shared; therefore, there is no communication overhead. On the other hand, there exist only a few efficient algorithms that address the scenario when the data is distributed (see~\cite{richtarik2013a},~\cite{Ravazzi2013}). Here, communication cost plays an important role and may have to be traded-off with per node computation cost. Furthermore, the optimization problem (\ref{minF}) can be solved in different ways depending on how the data is available per node~\cite{peng2013,boyd2011}: (1) example partition with all features, (2) feature partition with all examples and (3) combined example and feature partition (a block of examples/features). Methods such as distributed FISTA~\cite{peng2013} or ADMM~\cite{boyd2011} can be used when the data is example partitioned. In the combined partitioning case, methods such as block splitting~\cite{parikh2013} are useful. We are interested in the feature partitioning setting. 

In the algorithmic aspect, one important and popular category of methods is coordinate descent methods where a subset of variables are optimized at a time in an iterative fashion as given in Algorithm 1 until some convergence criterion is met. There are several key elements that need to be considered, and choices to be made for each one of them; they are: (i) selection of variables~\cite{tseng2009,yun2011}, (ii) approximation of the sub-problem objective function and its optimization for direction finding or weight update~\cite{beck2009,yun2011,yuan2012,fount2012,bryd2012}, (iii) line search (exact, approximate, no), (iv) conditions to be met to ensure (sufficient) decrease in the objective function value, in deterministic or expectation sense so that convergence guarantees can be given~\cite{nesterov2012,beck2009,yun2011,tseng2009, wang2013}, and, (5) acceleration mechanisms to improve the rate of convergence~\cite{beck2009,nesterov2012}. Yuan et al~\cite{yuan2012} studied various methods, specifically focusing on large scale linear classification problems with serial computations done in a single machine. Our interest is in comparing parallel/distributed computing methods. 

Parallel coordinate descent (PCD) methods can be grouped into methods that handle smooth and non-smooth objective functions. Since the $L1$ regularized loss function can be transformed to a smooth objective function in $2d$ variables with positivity constraints, PCD methods~\cite{neco2013,patriksson1998fp} that handle smooth objective functions are also of interest. We have seen how a generalized coordinate descent algorithm (Algorithm 1) can be written in a parallel/distributed computing setting involving the various elements (i)-(iv). So, we discuss how our work is similar to and different from other methods in the various elements; while Table 1 gives the summary, more details are presented below. \\ 

\subsection{P(D)CD Methods with $L1$ Regularized Sub-problems}

In this class of methods, the objective function of each sub-problem is written as the sum of a function that approximates the loss function and the regularizer term; therefore, it is still non-smooth. Due to the decomposable structure of the approximating function and the regularizer term, these sub-problems can be solved in parallel, and in some cases efficiently (e.g., closed form).  

\noindent{\bf Parallel Coordinate Descent Newton (PCDN)~\cite{bian2013}} Bian et al~\cite{bian2013} proposed a parallel coordinate descent method where randomized block partitioning of variables is done in each (outer) iteration. Then, each block of variables is sequentially optimized, and variables in each block are optimized in parallel using (diagonal) Hessian term in (\ref{quad}) followed by a line search. This line search is critical to achieve global convergence, and Bian et al. showed linear rate of convergence in the expectation sense (where expectation taken over the random partitioning of the variables). PCDN can be seen as a special case of the Algorithm 1 and our method; this follows from the generality of the algorithm with block coordinate optimization and various approximation function possibilities. We optimize per node block variables jointly, and perform line search across the blocks of variables; as the experimental results show, this can reduce the number of outer iterations significantly. Furthermore, we show global convergence and local linear rate of convergence in deterministic sense. \\

\noindent{\bf Distributed Coordinate Descent Method (DCDM)~\cite{richtarik2013a}} Richtarik and Takac~\cite{richtarik2013a} extended their initial work of parallel coordinate descent method~\cite{richtarik2013} suitable for multicore setting to the distributed setting. This method is closely related to ours and follows Algorithm 1, but differs from our method as indicated in Table 1. One key issue with this method is that setting the parameters $L^j$ accurately is a costly operation; on the other hand, inaccurate setting using cheaper computations results in slower convergence as our experiments show in Section~\ref{sec:motiv}. This also implies another level of trade-off in setting the parameters right to get improved efficiency. \\

\noindent{\bf Generic Coordinate Descent Method~\cite{scherrer2012a,scherrer2012}} Scherrer et al~\cite{scherrer2012a,scherrer2012} presented an abstract framework for coordinate descent methods (GenCD) suitable in parallel computing environments. In an extension, they introduced a randomized block greedy version and proved convergence results under certain descent conditions based on data properties. Several coordinate descent algorithms such as stochastic coordinate descent (SCD)~\cite{shwartz2011}, \textit{Shotgun}~\cite{bradley2011} and \textit{GRock}~\cite{peng2013} are covered by their method. Besides this, they suggested feature clustering before running the algorithm to improve efficiency, and discussed a \textit{thread greedy} selection of variables approach. We observe that GRock is a {thread greedy} algorithm in which the variables are selected greedily using gradient information. Note that feature clustering can be expensive, particularly, when data movement is needed in a distributed computing environment. Our algorithm (Algorithm 1) is similar to GenCD. However, besides the differences seen from Table 1, our method is targeted for the distributed computing environment involving communication (see for example, \textit{AllReduce} operation in step (d) of our algorithm). More importantly, algorithms such as \textit{Shotgun} and \textit{GRock} may not converge in practice due to their non-monotone nature; for example, we faced convergence issues on some datasets in our experiments with the GRock algorithm~\cite{peng2013}. Therefore, the practical utility of such algorithms is limited without ensuring necessary descent conditions.\\

\noindent{\bf Flexible Parallel Algorithms (FPA)~\cite{facchinei2013} } The FPA method~\cite{facchinei2013} has some similarities with our method in terms of the approximate function optimized at the nodes. But there are several fundamental differences between the methods. (a) FPA uses stochastic approximation step sizes instead of the line search used in our method. Because of this, FPA is a non-monotone method. As we will demonstrate in section x.y, there are serious practical issues associated with FPA's step size rules. (b) For our method, the proximal term merely plays a technical role for proving convergence. For example, when the loss function $f$ is strictly convex, our method can be shown to be convergent even without the proximal term. As we will show in section x.y, our method works very well even without the proximal term. On the other hand, the proximal term plays a crucial practical role for FPA. Tuning of the proximal parameter in FPA needs to be done carefully to get good efficiency. We will show in section x.y that the tuning idea outlined in~\cite{facchinei2013} is inadequate. (c) FPA does not address the issue of heavy communication costs in distributed solution. (d) The stopping condition used to stop the inner optimization of FPA is unverifiable; our method uses a verifiable relative condition. (e) When the loss is strictly convex, our method enjoys linear rate of convergence. This is not guaranteed for FPA. \\

\subsection{PCD Methods for Smooth Functions}
We briefly discuss two methods in this category. 

\noindent{\bf Synchronized Parallel Algorithm~\cite{patriksson1998fp}} Patriksson~\cite{patriksson1998} developed a cost approximation (CA) framework of descent algorithms for nonlinear optimization problems. He showed how a Jacobi type synchronous parallel algorithm with line search fits in this framework for differentiable objective functions~\cite{patriksson1998fp} over Cartesian product sets. When the CA functions (used to solve the direction finding sub-problems in parallel) are strongly convex, and additional conditions such as Armijo rule for line search step size selection and cyclic coordinate selection of variables are imposed, he proved linear rate of convergence. \\    

\noindent{\bf Parallel Block Coordinate Descent Method~\cite{neco2013}} Necora and Clipici~\cite{neco2013} proposed an iterative algorithm where they solved (\ref{quad}) for all coordinates (block wise) in parallel, using coordinate Lipschitz constants for the gradient. The weights are updated in parallel as a weighted combination of previous weight and the incremental update obtained from solving (\ref{quad}). They showed sub-linear and linear rate of convergence results without and with strong convexity assumption. \\

\subsection{ADMM Methods}

%\item Efficient parallel coordinate descent algorithm for convex optimization problems with separable constraints: application to distributed MPC (Necoara and Clipici, 2013). 

\begin{itemize}
\item Accelerated ADMM 
\item On the $O(\frac{1}{k})$ convergence and parallelization of the ADMM (Deng et al, 2013). 
\end{itemize}


\begin{table*}
\centering
\caption{{\scriptsize Properties of Various Methods. $*$ indicates monotone in the expectation sense for certain combination of sampling types and constants $L_i$ settings. $+$ indicates distributed versions (like our method) implemented in our experiments. $\dagger$ indicates convergence only under certain conditions on the spectral radius of data matrix. $\triangle$ represents the class of smooth function optimization and all variables are updated in parallel; variants are possible. The descent and convergence rate (sub-linear/linear) results are dependent on conditions such as (strong) convexity of the approximating functions, Lipschitz continuous gradient, line search step size and variable selection rules. The variables in the sub-problem are jointly optimized only in our method.}}
{\small
\begin{tabular}{|p{1.85cm}|p{1.75cm}|p{2cm}|p{1.75cm}|p{1.75cm}|p{2cm}|p{1.75cm}|} \hline
Method & F behavior (descent) & Feature limit/selection & Proximal term & Line search & Convergence & Rate of convergence \\ \hline
Bradley~et~al~\cite{bradley2011} & Non-monotone & Limited /Random & Lipschitz & None & In expectation & Sub-linear$^\dagger$ \\ \hline
Richtarik and Takac~\cite{richtarik2012} & Monotone$^*$ & No~limits /Random & Maximal bound & None & In expectation & Linear \\ \hline
Richtarik and Takac~\cite{richtarik2013}$^+$ & Monotone$^*$ & No~limits /Random & Maximal bound & None & In expectation & Linear \\ \hline
GRock~\cite{peng2013}$^{+}$ & Non-monotone & Limited /Greedy & Lipschitz & None & None & Sub-linear$^\dagger$ \\ \hline
PCDN~\cite{bian2013}$^+$ & Descent & No~limits /Random & Hessian diagonals & Armijo & In Expectation & Linear \\ \hline
PCD~\cite{neco2013}$^\triangle$ & Descent & Full & Lipschitz & None & Deterministic & Linear \\ \hline  
SPA~\cite{patriksson1998fp}$^\triangle$ & Descent & Full & Lipschitz & Armijo & Deterministic & Linear \\ \hline  
Our method & Descent & No~limits /Random or Greedy & Free & Armijo & Deterministic & Linear \\ \hline
\end{tabular}
}
\end{table*}


